Effect of triangularity on plasma turbulence and the SOL-width scaling in L-mode diverted tokamak configurations

The effect of triangularity on tokamak boundary plasma turbulence is investigated by using global, flux-driven, three-dimensional, two-fluid simulations. The simulations show that negative triangularity stabilizes boundary plasma turbulence, and linear investigations reveal that this is due to a reduction of the magnetic curvature drive of interchange instabilities, such as the resistive ballooning mode. As a consequence, the pressure decay length $L_p$, related to the SOL power fall-off length $\lambda_q$, is found to be affected by triangularity. Leveraging considerations on the effect of triangularity on the linear growth rate and nonlinear evolution of the resistive ballooning mode, the analytical theory-based scaling law for $L_p$ in L-mode plasmas, derived by Giacomin \textit{et al.} [{Nucl. Fusion}, \href{https://doi.org/10.1088/1741-4326/abf8f6}{\textbf{61} 076002} (2021)], is extended to include the effect of triangularity. The scaling is in agreement with nonlinear simulations and a multi-machine experimental database, which include recent TCV discharges dedicated to the study of the effect of triangularity in L-mode diverted discharges. Overall, the present results highlight that negative triangularity narrows the $L_p$ and considering the effect of triangularity is important for a reliable extrapolation of $\lambda_q$ from present experiments to larger devices.

==> 9_bib.tex <==
@article{Halpern2016,
    author = "Halpern, F. C. and others",
    title = "The {GBS} code for tokamak scrape-off layer simulations",
    journal = "J. Comput. Phys.",
    volume =  "\href{https://doi.org/10.1016/j.jcp.2016.03.040}
    {\textbf{315} 388}",
    year = {(2016)},
}

@article{Paruta2018,
    author = {Paruta, P. and others},
    title = {Simulation of plasma turbulence in the periphery of diverted tokamak by using the {GBS} code},
    journal = {Phys. Plasmas},
    volume =  "\href{https://doi.org/10.1063/1.5047741}
    {\textbf{25} 112301}",
    year = {(2018)},
}

@article{Wersal2015,
    author = "Wersal, C. and Ricci, P",
    title = "{A first-principles self-consistent model of plasma turbulence and kinetic neutral dynamics in the tokamak scrape-off layer}",
    journal = "Nucl. Fusion",
    volume =  "\href{https://doi.org/10.1088/0029-5515/55/12/123014}
    {\textbf{55} 123014}",
    year = {(2015)},
}

@article{Zeiler1997,
    author = {Zeiler,A.  and Drake,J. F.  and Rogers,B.},
    title = {{Nonlinear reduced Braginskii equations with ion thermal dynamics in toroidal plasma}},
    journal = {Phys. Plasams},
    volume =  {\href{https://doi.org/10.1063/1.872368}
    {\textbf{4} 2134}},
    year = {(1997)}},
}

@article{Morales2016,
    author = "Morales, J. and others",
    title = "{The impact of the Boussinesq approximation on plasma turbulence in the scrape-off layer}",
    journal = "Eurofusion",
    year = {(2016)}},
}

@article{Bodi2011,
    author = "Bodi, K. and others",
    title = "{Impact of the Boussinesq approximation in tokamak scrape-off layer}",
    journal = "38th EPS conference",
    volume =  "P1.121",
    year = {(2011)}},
}

@article{Manz2015,
    author = {Manz, P. and others},
    title = {Origin and turbulence spreading of plasma blobs},
    journal = {Phys. Plasmas},
    volume =  "\href{https://doi.org/10.1063/1.4908272}
    {\textbf{22} 022308}",
    year = {(2015)},
}

@article{Xu2009,
    author = {Xu, G. S. and others},
    title = {Blob/hole formation and zonal-flow generation in the edge plasma of the 1JET tokamak},
    journal = {Nucl. Fusion},
    volume =  "\href{https://doi.org/10.1088/0029-5515/49/9/092002}
    {\textbf{49} 092002}",
    year = "2009",
}

@article{Happel2009,
  title = {Generation of Intermittent Turbulent Events at the Transition from Closed to Open Field Lines in a Toroidal Plasma},
  author = {Happel, T. and Greiner, F. and Mahdizadeh, N. and Nold, B. and Ramisch, M. and Stroth, U.},
  journal = {Phys. Rev. Lett.},
  volume =  "\href{https://10.1103/PhysRevLett.102.255001}{\textbf{25} 255001}",
  year = {(2009)},
}

@article{Krasheninnikov2008,
  title = {Dynamics and generation mechanisms of mesoscale structures in tokamak edge plasmas},
  author = {Krasheninnikov, S. I. and Smolyakov, A. I.},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.2896570}{\textbf{15} 055909}",
  year = {(2008)},
}

@article{Riva2017,
    title = {Plasma shaping effects on tokamak scrape-off layer turbulence},
    author = {Riva, F. and Lanti, E and Jolliet, S. and Ricci, P.},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/1361-6587/aa5322}{\textbf{59} 035001}},
    year = {(2017)},
}

@article{Riva2020,
  title = {Shaping effects on scrape-off layer plasma turbulence: A rigorous validation of three-dimensional simulations against TCV measurements},
  author = {Riva, F. and others},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.5123451}{\textbf{27} 012301}",
  year = {(2020)},
}

@article{Marinoni2021,
    title = {A brief history of negative triangularity tokamak plasmas},
    author = {Marinoni, A. and Sauter, O. and Coda, S.},
    journal = {Rev. Mod. Plasma Phys.},
    volume =  {\href{https://doi.org/10.1007/s41614-021-00054-0}{\textbf{5} 6}},
    year = {(2021)},
}

@article{Han2021,
  title = {Suppression of first-wall interaction in negative triangularity plasmas on {TCV}},
  author = {Han, W. and others},
  journal = {Nucl. Fusion},
  volume =  "\href{https://doi.org/10.1088/1741-4326/abdb95}{\textbf{61} 034001}",
  year = {(2021)},
}

@phdthesis{Baudoin2018,
  author       = {Camille Baudoin}, 
  title        = {Numerical evaluations of mechanisms governing the heat transport in the edge plasma of tokamaks},
  school       = {Aix-Marseille University},
  year         = {(2018)},
}

@article{Halpern2013,
  title = {Theory-based scaling of the {SOL} width in circular limited tokamak plasmas},
  author = {Halpern, F. D. and others},
  journal = {Nucl. Fusion},
  volume =  "\href{https://doi.org/10.1088/0029-5515/53/12/122001}{\textbf{53} 122001}",
  year = {(2013)},
}

@article{Halpern2014,
  title = {Theory of the scape-off layer width in inner-wall limited tokamak plasmas},
  author = {Halpern, F. D. and others},
  journal = {Nucl. Fusion},
  volume =  "\href{https://doi.org/10.1088/0029-5515/54/4/043003}{\textbf{54} 043003}",
  year = {(2014)},
}

@article{Ricci2013,
  title = {Plasma turbulence in the scrape-off layer of tokamak devices},
  author = {Ricci, P. and Rogers, B. N.},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.4789551}{\textbf{20} 010702}",
  year = {(2013)},
}

@article{Ricci2008,
  title = {High- and Low-Confinement Modes in Simple Magnetized Toroidal Plasmas},
  author = {Ricci, P. and Rogers, B. N. and Brunner, S.},
  journal = {Phys. Rev. Lett.},
  volume =  "\href{https://doi.org/10.1103/PhysRevLett.100.225002}{\textbf{100} 225002}",
  year = {(2008)},
}

@article{Mosetto2012,
  title = {Low-frequency linear-mode regimes in the tokamak scrape-off layer},
  author = {Mosetto, A. and others},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.4758809
}{\textbf{19} 112103}",
  year = {(2012)},
}

@article{Mosetto2013,
  title = {Turbulent regimes in the tokamak scrape-off layer},
  author = {Mosetto, A. and others},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.4821597}{\textbf{20} 092308}",
  year = {(2013)},
}

@article{Merlo2019,
  title = {Turbulent transport in {TCV} plasmas with positive and negative triangularity},
  author = {Merlo, G. and others},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.5115390}{\textbf{26} 102302}",
  year = {(2019)},
}

@article{Laribi2021,
    title = {Impact of negative triangularity on edge plasma transport and turbulence in {TOKAMAK3X} simulations},
    author = {E. Laribi and E. Serre and P. Tamain and H. Yang},
    journal = {Nucl. Mater. Energy},
    volume =  {\href{https://doi.org/10.1016/j.nme.2021.101012}{\textbf{27} 101012}},
    year = {(2021)},
}

@article{Beadle2020,
    title = {Understanding the turbulent mechanisms setting the density decay length in the tokamak scrape-off layer},
    author = {Beadle, C. and Ricci, P},
    journal = {J. Plasma Phys.},
    volume =  {\href{https://doi.org/10.1017/S0022377820000094}{\textbf{86} 175860101}},
    year = {(2020)},
}

@article{Rafiq2010,
  title = {Development of drift-resistive-inertial ballooning transport model for tokamak edge plasmas},
  author = {Rafiq, T. and others},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.3478979}{\textbf{17} 082511}",
  year = {(2010)},
}

@article{Connor1978,
    title = {{Shear, periodicity, and plasma ballooning modes}},
    author = {Connor, J. W. and Hastie, R. J. and Taylor, J. B.},
    journal = {Phys. Rev. Lett.},
    volume =  "\href{https://doi.org/10.1103/PhysRevLett.40.396}{\textbf{40} 396}",
    year = {1978},
}

@article{Bateman1978,
  title = {Resistive-Ballooning-Mode Equation},
  author = {Bateman, G. and Nelson, D.B.},
  journal = {Phys. Rev. Lett.},
  volume =  "\href{https://doi.org/10.1103/PhysRevLett.41.1804}{\textbf{41} 1804}",
  year = {1978},
}

@article{McCarthy1992,
  title = {{Stability of resistive and ideal ballooning modes in the Texas Experimental Tokamak and DIII‐D}},
  author = {McCarthy, D.R. and others},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.860038}{\textbf{4} 1846}",
  year = {1992},
}

@article{Novakovskii1995,
  title = {{New unstable branch of drift resistive ballooning modes in tokamaks}},
  author = {Novakovskii, S.V. and others},
  journal = {Phys. Plasmas},
  volume =  {\href{https://doi.org/10.1063/1.871431}{\textbf{2} 781}},
  year = {1995},
}

@article{Mima1978,
author = {Mima, Kunioki and Hasegawa, Akira},
journal = {Phys. Fluids},
title = {{Nonlinear instability of electromagnetic drift waves}},
volume =  {\href{https://doi.org/10.1063/1.862082}{\textbf{21} 81}},
year = {1978}
}

@article{Wakatani1984,
author = {Wakatani, Masahiro and Hasegawa, Akira},
doi = {10.1063/1.864660},
journal = {Phys. Fluids},
title = {{A collisional drift wave description of plasma edge turbulence}},
volume =  {\href{https://doi.org/10.1063/1.864660}{\textbf{27} 611}},
year = {1984}
}

@article{Sugama1988,
   author = {Hideo Sugama and Masahiro Wakatani and Akira Hasegawa},
   doi = {10.1063/1.866699},
   issn = {00319171},
   issue = {6},
   journal = {Phys. Fluids},
   title = {Study of resistive drift and resistive interchange modes in a cylindrical plasma with magnetic shear},
   volume =  {\href{https://doi.org/10.1063/1.866699}{\textbf{31} 1601}},
   year = {1988},
}

@article{Horton1999,
   author = {W. Horton},
   doi = {10.1103/revmodphys.71.735},
   journal = {Rev. Mod. Phys.},
   title = {Drift waves and transport},
   volume =  {\href{https://doi.org/10.1103/revmodphys.71.735}{\textbf{71} 735}},   
   year = {1999},
}

@article{Diamond2011,
   author = {P. H. Diamond and A. Hasegawa and K. Mima},
   doi = {10.1088/0741-3335/53/12/124001},
   journal = {Plasma Phys. Control. Fusion},
   title = {Vorticity dynamics, drift wave turbulence, and zonal flows: a look back and a look ahead},
   volume =  {\href{https://doi.org/10.1088/0741-3335/53/12/124001}{\textbf{53} 124001}},
   year = {2011},
}

@book{Dhaeseleer1991,
   author = {W. D. D’haeseleer and William Nicholas Guy Hitchon and James D. Callen and J. Leon Shohet},
   ISBN = {10.1007/978-3-642-75595-8},
   publisher = {Springer Berlin Heidelberg},
   title = {Flux Coordinates and Magnetic Field Structure},
   year = {(1991)},
}

@article{Moret1997,
author = {Moret, J. M. and Franke, S. and Weisen, H. and Anton, M. and Behn, R. and Duval, B. P. and Hofmann, F. and Joye, B. and Martin, Y. and Nieswand, C. and Pietrzyk, Z. A. and van Toledo, W.},
doi = {10.1103/PhysRevLett.79.2057},
journal = {Phys. Rev. Lett.},
title = {{Influence of plasma shape on transport in the TCV tokamak}},
volume =  {\href{https://doi.org/10.1103/PhysRevLett.79.2057}{\textbf{79} 2057}},
year = {1997}
}

@article{Sauter1999,
author = {Sauter, O. and Angioni, C. and Lin-Liu, Y. R.},
doi = {10.1063/1.873240},
journal = {Phys. Plasmas},
title = {{Neoclassical conductivity and bootstrap current formulas for general axisymmetric equilibria and arbitrary collisionality regime}},
volume =  {\href{https://doi.org/10.1063/1.873240}{\textbf{6} 2834}},
year = {1999}
}

@article{Austin2019,
author = {Austin, M. E. and others},
doi = {10.1103/PhysRevLett.122.115001},
journal = {Phys. Rev. Lett.},
publisher = {American Physical Society},
title = {{Achievement of Reactor-Relevant Performance in Negative Triangularity Shape in the DIII-D Tokamak}},
url = {https://doi.org/10.1103/PhysRevLett.122.115001},
volume =  {\href{https://doi.org/10.1103/PhysRevLett.122.115001}{\textbf{122} 115001}},
year = {(2019)}
}

@article{Kikuchi2019,
author = {Kikuchi, M. and others},
doi = {10.1088/1741-4326/ab076d},
journal = {Nucl. Fusion},
title = {{L-mode-edge negative triangularity tokamak reactor}},
volume =  {\href{https://doi.org/10.1088/1741-4326/ab076d}{\textbf{59} 056017}},
year = {(2019)}
}

@article{Medvedev2015,
author = {Medvedev, S. and others},
doi = {10.1088/0029-5515/55/6/063013},
journal = {Nucl. Fusion},
number = {6},
title = {{The negative triangularity tokamak: Stability limits and prospects as a fusion energy system}},
volume =  {\href{https://doi.org/10.1088/0029-5515/55/6/063013}{\textbf{55} 063013}},
year = {(2015)}
}

@article{Marinoni2009,
author = {Marinoni, A. and others},
doi = {10.1088/0741-3335/51/5/055016},
issn = {07413335},
journal = {Plasma Phys. Control. Fusion},
number = {5},
title = {{The effect of plasma triangularity on turbulent transport: Modeling TCV experiments by linear and non-linear gyrokinetic simulations}},
volume =  {\href{https://doi.org/10.1088/0741-3335/51/5/055016}{\textbf{51} 055016}},
year = {(2009)}
}

@article{Reimerdes2000,
    author = {Reimerdes, H. and Pochelon, A. and Sauter, O. and Goodman, T. P. and Henderson, M. A. and Martynov, An},
    doi = {10.1088/0741-3335/42/6/302},
    journal = {Plasma Phys. Control. Fusion},
    pages = {629},
    title = {{Effect of triangular and elongated plasma shapeon the sawtooth stability}},
    volume =  {\href{https://doi.org/10.1088/0741-3335/42/6/302}{\textbf{42} 629}},
    year = {(2000)}
}

@article{Camenen2007,
    author = {Camenen, Y. and others},
    doi = {10.1088/0029-5515/47/7/002},
    journal = {Nucl. Fusion},
    title = {{Impact of plasma triangularity and collisionality on electron heat transport in TCV L-mode plasmas}},
    volume =  {\href{https://doi.org/10.1088/0029-5515/47/7/002}{\textbf{47} 510}},
    year = {(2007)}
}

@article{Kikuchi2014,
author = {Kikuchi, M. and others},
doi = {10.3390/ECE-1-E002},
journal = {Proceedings of 1st International e-Conference on Energies},
title = {{Negative Triangularity Tokamak as Fusion Energy System}},
volume =  {\href{https://doi.org/10.3390/ECE-1-E002}{\textbf{1} E002}},
year = {(2014)}
}

@article{Fontana2018,
author = {Fontana, M. and Porte, L. and Coda, S. and Sauter, O.},
doi = {10.1088/1741-4326/AA98F4},
journal = {Nucl. Fusion},
title = {{The effect of triangularity on fluctuations in a tokamak plasma}},
volume =  {\href{https://doi.org/10.1088/1741-4326/AA98F4}{\textbf{58} 024002}},
year = {(2018)}
}

@article{Marinoni2019,
author = {Marinoni, A. and others},
doi = {10.1063/1.5091802},
journal = {Phys. Plasmas},
title = {{H-mode grade confinement in L-mode edge plasmas at negative triangularity on DIII-D}},
volume =  {\href{https://doi.org/10.1063/1.5091802}{\textbf{26} 042515}},
year = {(2019)}
}

@article{Huang2019,
    author = {Huang, Z. and Coda, S. and the TCV team},
    doi = {10.1088/1361-6587/aadb59},
    journal = {Plasma Phys. Control. Fusion},
    title = {{Dependence of density fluctuations on shape and collisionality in positive- and negative-triangularity tokamak plasmas}},
    volume =  {\href{https://dx.doi.org/10.1088/1361-6587/aadb59}{\textbf{61} 014921}},
    year = {(2019)}
}

@article{Austin2018,
author = {Austin, M. E. and others},
doi = {10.1088/1361-6587/aadb59},
journal = {27th IAEA Fusion Energy Conference (FEC 2018)},
title = {{High confinement in negative triangularity discharges in DIII-D}},
volume =  {IAEA-CN--258},
year = {(2018)}
}

@article{Marinoni2021_2,
author = {Marinoni, A. and others},
doi = {https://doi.org/10.1088/1741-4326/ac1f60},
journal = {Nucl. Fusion},
title = {{Diverted negative triangularity plasmas on DIII-D: the benefit of high confinement without the liability of an edge pedestal}},
volume =  {\href{https://doi.org/10.1088/1741-4326/ac1f60}{\textbf{61} 116010}},
year = {(2021)}
}

@article{Merlo2021,
  title = {Nonlocal effects in negative triangularity {TCV} plasmas},
  author = {Merlo, G. and others},
  journal = {Plasma Phys. Control. Fusion},
  volume =  "\href{https://doi.org/10.1088/1361-6587/abe39d}{\textbf{63} 044001}",
  year = {(2021)},
}

@article{Merlo2015,
  title = {Investigating profile stiffness and critical gradients in shaped TCV discharges using local gyrokinetic simulations of turbulent transport},
  author = {Merlo, G. and others},
  journal = {Plasma Phys. Control. Fusion},
  volume =  "\href{https://doi.org/10.1088/0741-3335/57/5/054010}{\textbf{57} 054010}",
  year = {(2015)},
}

@article{Rewoldt1982,
   author = {G. Rewoldt and W. M. Tang and M. S. Chance},
   journal = {Phys. Fluids},
   title = {Electromagnetic kinetic toroidal eigenmodes for general magnetohydrodynamic equilibria},
   volume =  "\href{https://doi.org/10.1063/1.863760}{\textbf{25} 480}",
   year = {(1982)},
}

@article{Kinsey2007,
  title = {The effect of plasma shaping on turbulent transport and $E \times B$ shear quenching in nonlinear gyrokinetic simulations},
  author = {Kinsey, J. E. and Waltz, R. E. and Candy, J.},
  journal = {Phys. Plasmas},
  volume =  "\href{https://doi.org/10.1063/1.2786857}{\textbf{14} 102306}",
  year = {(2007)},
}

@article{Luce2013,
  title = {An analytic functional form for characterization and generation of axisymmetric plasma boundaries},
  author = {Luce, T.},
  journal = {Plasma Phys. Control. Fusion},
  volume =  "\href{https://doi.org/10.1088/0741-3335/55/9/095009}{\textbf{55} 095009}",
  year = {(2013)},
}

@article{Camenen2005,
  title = {{Electron heat transport in shaped TCV L-mode plasmas}},
  author = {Camenen, Y. and others},
  journal = {Plasma Phys. Control. Fusion},
  volume =  "\href{https://doi.org/10.1088/0741-3335/47/11/007}{\textbf{47} 1971}",
  year = {(2005)},
}

@article{Stober2000,
   author = {J Stober and O Gruber and A Kallenbach and V Mertens and F Ryter and A Stäbler and W Suttrop and W Treutterer and the ASDEX Upgrade Team},
   doi = {10.1088/0741-3335/42/5A/324},
   journal = {Plasma Phys. Control. Fusion},
   title = {Effects of triangularity on confinement, density limit and profile stiffness of H-modes on ASDEX upgrade},
   volume =  "\href{https://doi.org/10.1088/0741-3335/42/5A/324}{\textbf{42} A211}",
   year = {(2000)},
}

@article{Saibene2002,
   author = {G Saibene and R Sartori and A Loarte and D J Campbell and P J Lomas and V Parail and K D Zastrow and Y Andrew and S Sharapov and A Korotkov and M Becoulet and G T A Huysmans and H R Koslowski and R Budny and G D Conway and J Stober and W Suttrop and A Kallenbach and M von Hellermann and M Beurskens},
   journal = {Plasma Phys. Control. Fusion},
   title = {{Improved performance of ELMy H-modes at high density by plasma shaping in JET}},
   volume =  "\href{https://doi.org/10.1088/0741-3335/44/9/301}{\textbf{44} 1769}",
   year = {(2002)},
}

@article{Schoepf2001,
   author = {Schoepf, K. and others},
   journal = {Unknown, see google drive},
   title = {{Effects of tokamak flux surface non-circularity on charged particle transport in the weak collisionality regime}},
   volume =  {\href{https://doi.org/10.1088/0741-3335/44/9/301}{\textbf{44} 1769}},
   year = {(2001)},
}


@article{Fontana2020,
    author = {Fontana, M. and others},
    journal = {Nucl. Fusion},
    title = {{Effects of collisionality and $T_e/T_i$ on fluctuations in positive and negative tokamak plasmas}},
    volume =  {\href{https://doi.org/10.1088/1741-4326/ab4d75}{\textbf{60} 016006}},
    year = {(2020)}
}

@article{Editors1999,
author = {Editors, ITER Physics Basis and an Co-Chairs, ITER Physics Expert Group Chairs and Unit, ITER Joint Central Team and Physics},
journal = {Nucl. Fusion},
title = {{Chapter 1: Overview and summary}},
volume =  {\href{https://doi.org/10.1088/0029-5515/39/12/301}{\textbf{39} 2137}},
year = {(1999)}
}

@article{Coda2022,
author = {S. Coda and others},
journal = {Plasma Phys. Control. Fusion},
title = {{Enhanced confinement in diverted negative-triangularity L-mode plasmas in TCV}},
volume =  {\href{https://doi.org/10.1088/1361-6587/ac3fec}{\textbf{64} 014004}},
year = {(2022)}
}

@article{Song2021,
author = {Junhyuk Song and Carlos Paz-Soldan and Jungpyo Lee},
journal = {Nucl. Fusion},
title = {{Impact of negative triangularity plasma shaping on the n = 0 resistive wall mode in a tokamak}},
volume =  {\href{https://doi.org/10.1088/1741-4326/ac189a}{\textbf{61} 096033}},
year = {(2021)}
}

@article{Lomas2000,
author = {P J Lomas and on behalf of the JET Joint Undertak Team},
journal = {Plamsa Phys. Cont. Fusion},
title = {{The variation of confinement with elongation and triangularity in {ELMy} H-modes on {JET}}},
volume =  {\href{https://doi.org/10.1088/0741-3335/42/12b/309}{\textbf{42} B115}},
year = {(2000)}
}

@article{Yushmanov1990,
author = {P.N. Yushmanov and T. Takizuka and K.S. Riedel and O.J.W.F. Kardaun and J.G. Cordey and S.M. Kaye and D.E. Post},
journal = {Nucl. Fusion},
title = {{Scalings for tokamak energy confinement}},
volume =  {\href{https://doi.org/10.1088/0029-5515/30/10/001}{\textbf{30} 1999}},
year = {(1990)}
}

@article{Johner2011,
author = {J. Johner},
journal = {Fusion Sci. Technol.},
title = {{HELIOS: A Zero-Dimensional Tool for Next Step and Reactor Studies}},
volume =  {\href{https://doi.org/10.13182/FST11-A11650}{\textbf{59} 308}},
year = {(2011)}
}

@article{Kikuchi2014_2,
author = { Mitsuru Kikuchi and  Tomonori Takizuka and  Masaru Furukawa},
journal = {JPS Conf. Proc.},
title = {Negative Triangularity as a Possible Tokamak Scenario},
year= {(2014)},
volume =  {\href{https://doi.org/10.7566/JPSCP.1.015014}{\textbf{1} 015014}}
}

@article{Pochelon1999,
    author = {A Pochelon and others},
    journal = {Nucl. Fusion},
    title = {Energy confinement and {MHD} activity in shaped {TCV} plasmas with localized electron cyclotron heating},
	volume =  {\href{https://doi.org/10.1088/0029-5515/39/11y/321}{\textbf{39} 1807}},
	year = {(1999)}
}


@article{Sauter2016,
    author = {O. Sauter},
    journal = {Fusion Eng. Des.},
    title = {Geometric formulas for system codes including the effect of negative triangularity},
	volume =  {\href{https://doi.org/10.1016/j.fusengdes.2016.04.033}{\textbf{112} 633}},
	year = {(2016)}
}

@article{Faitsch2018,
    author = {M. Faitsch and others},
    journal = {Plasma Phys. Control. Fusion},
    title = {{Dependence of the L-Mode scrape-off layer power fall-off length on the upper triangularity in TCV}},
	volume =  {\href{https://doi.org/10.1088/1361-6587/aaaef7}{\textbf{60} 045010}},
	year = {(2018)}
}

@article{Giacomin2022,
    author = {M. Giacomin and others},
    journal = {J. Comput. Phys.},
    title = {{The GBS code for the self-consistent
    simulation of plasma turbulence and kinetic neutral dynamics in the tokamak boundary}},
    volume =  {\href{https://doi.org/10.1016/j.jcp.2022.111294}{\textbf{463} 111294}},
	year = {(2022)},
}

@article{Giacomin2020,
    author = {M. Giacomin and P. Ricci},
    journal = {J. Plasma Phys.},
    title = {{Investigation of turbulent transport regimes in the tokamak edge by using two-fluid simulations}},
    volume =  {\href{https://doi.org/10.1017/S0022377820000914}{\textbf{5} 86}},
	year = {(2020)}
}

@article{Giacomin2020_2,
    author = {M. Giacomin and L.N. Stenger and P. Ricci},
    journal = {Nucl. Fusion},
    title = {{Turbulence and flows in the plasma boundary of snowflake magnetic configurations}},
    volume =  {\href{https://doi.org/10.1088/1741-4326/ab6435}{\textbf{60} 024001}},
	year = {(2020)}
}

@article{Weisen1997,
    author = {H. Weisen and others},
    journal = {Nucl. Fusion},
    title = {{Effect of plasma shape on confinement and MHD behaviour in the TCV tokamak}},
    volume =  {\href{https://doi.org/10.1088/0029-5515/37/12/I07}{\textbf{37} 1741}},
	year = {(1997)}
}

@article{Loizu2012,
    author = {J. Loizu and P. Ricci and F. D. Halpern and S. Jolliet},
    journal = {Phys. Plasmas},
    title = {{Boundary conditions for plasma fluid models at the magnetic presheath entrance}},
    volume =  {\href{https://doi.org/10.1063/1.4771573}{\textbf{19} 122307}},
	year = {(2012)}
}

@article{Graves2013,
    author = {J. P. Graves},
    journal = {Plasma Phys. Control. Fusion},
    title = {{Toroidal drift precession and wave–particle interaction in shaped tokamaks with finite beta and neoclassical equilibrium effects}},
    volume =  {\href{https://doi.org/10.1088/0741-3335/55/7/074009}{\textbf{55} 074009}},
	year = {(2013)}
}

@article{Madden1994,
    author = {N.A Madden and R.J Hastie},
    journal = {Nucl. Fusion},
    title = {{Tokamak equilibrium with anisotropic pressure}},
    volume =  {\href{https://doi.org/10.1088/0029-5515/34/4/i05}{\textbf{34} 519}},
	year = {(1994)}
}

@article{Duff2022,
    author = {Duff,J. M.  and Faber,B. J.  and Hegna, C. C.  and Pueschel, M. J.  and Terry, P. W. },
    journal = {Phys. Plasmas},
    title = {{Effect of triangularity on ion-temperature-gradient-driven turbulence}},
    volume =  {\href{https://doi.org/10.1063/5.0065585}{\textbf{29} 012303}},
	year = {(2022)}
}

@article{Faitsch2015,
	author = {M. Faitsch and B. Sieglin and T. Eich and H. J. Sun and A. Herrmann and the ASDEX Upgrade Team},
	title = {{Change of the scrape-off layer power width with the toroidal B-field direction in {ASDEX} upgrade}},
	journal = {Plasma Phys. Control. Fusion},
	volume =  {\href{https://doi.org/10.1088/0741-3335/57/7/075005}{\textbf{57} 075005}},
	year = {(2015)},
}

@article{Goldston2011,
author = {Goldston, R.J.},
journal = {Nucl. Fusion},
title = {{Heuristic drift-based model of the power scrape-off width in low-gas-puff H-mode tokamaks}},
volume =  {\href{https://doi.org/10.1088/0029-5515/52/1/013009}{\textbf{52} 013009}},
year = {(2011)}
}

@article{Fundamenski2005,
author = {W. Fundamenski and P. Andrew and K. Erents and A. Huber and G. Kirnev and G. Matthews and R. Pitts and V. Riccardo and S. Sipilä},
title = {{Effect of $B\times \nabla B$ direction on SOL energy transport in JET}},
volume =  {\href{https://doi.org/10.1016/j.jnucmat.2004.08.030}{\textbf{337-339} 305}},
year = {(2011)},
}

@article{Wan2015,
author = {Wan, W.  and Chen,Y.  and Parker,S.  and Groebner,R. J. },
title = {Effects of the magnetic equilibrium on gyrokinetic simulations of tokamak microinstabilities},
journal = {Phys. Plasmas},
volume =  {\href{https://doi.org/10.1063/1.4922079}{\textbf{22} 062502}},
year = {(2015)},
}

@article{Lao2001,
    author = {L.L Lao and others},
    title = {Dependence of edge stability on plasma shape and local pressure gradients in the {DIII-D} and {JT-60U} tokamaks},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/41/3/306}{\textbf{41} 295}},
	year = {(2001)},
}

@article{Crisanti2003,
    author = {F Crisanti and others},
    title = {Role of the plasma shaping in {ITB} experiments on {JET}},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/0741-3335/45/4/305}{\textbf{45} 379}},
	year = {(2003)},
}

@article{Giacomin2021_2,
author = {Giacomin, M. and others},
title = {{Theory-based scaling laws of near and far scrape-off layer widths in single-null L-mode discharges}},
journal = {Nucl. Fusion},
volume =  {\href{https://doi.org/10.1088/1741-4326/abf8f6}{\textbf{61} 76002}},
year = {(2021)},
}

@article{Giacomin2022_2,
    author = {Giacomin, M. and Ricci,P. },
    title = {Turbulent transport regimes in the tokamak boundary and operational limits},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/5.0090541}{\textbf{29} 062303}},
    year = {(2022)},
}



@article{Horacek2020,
	author = {J. Horacek and others},
	title = {{Scaling of L-mode heat flux for ITER and COMPASS-U divertors, based on five tokamaks}},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/1741-4326/ab7e47}{\textbf{60} 066016}},
    year = {(2020)},
}

@article{Jean2011,
  title = {{HELIOS: A zero-dimensional tool for next step and reactor studies}},
  author = {J. Johner},
  journal = {Fusion Sci. Technol.},
  volume =  "\href{https://doi.org/10.13182/FST11-A11650
}{\textbf{59} 308}",
  year = {(2011)},
}

@article{Loarte2007,
    author = {A. Loarte and others},
    title = {Chapter 4: Power and particle control},
	volume =  "\href{https://doi.org/10.1088/0029-5515/47/6/s04}{\textbf{47} S203}",
	journal = {Nucl. Fusion},
	year = {(2007)},
}

@article{Jolliet2014,
    author = {Jolliet, S. and Halpern, F. D.  and Loizu, J. and Mosetto, A. and Ricci, P.},
    title = {Aspect ratio effects on limited scrape-off layer plasma turbulence},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.4863956}{\textbf{21} 022303}},
    year = {(2014)},
}

@article{Coelho2022,
	author={Coelho, A. and Loizu, J. and Ricci, P. and Giacomin, M.},
	title={Global fluid simulation of plasma turbulence in a stellarator with an island divertor},
	journal={Nucl. Fusion},
	volume =  {\href{https://dx.doi.org/10.1088/1741-4326/ac6ad2}{\textbf{62} 074004}},
	year={(2022)},
}

@article{Mancini2021,
    author = {D. Mancini and P. Ricci and N. Vianello and M. Giacomin and A. Coroado},
	title = {Investigation of the density shoulder formation by using self-consistent simulations of plasma turbulence and neutral kinetic dynamics},
	volume =  "\href{https://doi.org/10.1088/1741-4326/ac30c9}{\textbf{61} 126029}",	
	journal = {Nucl. Fusion},
	year = {(2021)},
}

@article{Lazarus1991,
    author = {Lazarus, E. A. and others},
    title = {Higher beta at higher elongation in the {DIII‐D} tokamak},
    journal = {Phys. Fluids B},
    volume =  "\href{https://doi.org/10.1063/1.859639}{\textbf{3} 2220}",
    year = {(1991)},
}

@article{Miura1992,
    author = {Y. Miura and others},
	title = {Geometric dependence of the energy confinement time scaling for {H}-mode discharges},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/0029-5515/32/8/i15}{\textbf{32} 1473}},
	year = {(1992)},
}

@article{Ippolito2011,
    author = {D’Ippolito,D. A.  and Myra,J. R.  and Zweben,S. J. },
    title = {{Convective transport by intermittent blob-filaments: Comparison of theory and experiment}},
    journal = {Phys. Plasmas},
    volume =  "\href{https://doi.org/10.1063/1.3594609}{\textbf{18} 060501}",
    year = {(2011)},
}

@article{Kendl2006,
    author = {Kendl, A.  and Scott,B. D. },
    title = {Flux-surface shaping effects on tokamak edge turbulence and flows},
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.2158695}{\textbf{13} 012504}},
    year = {(2006)},
}

@article{Scott1997,
    author = {B. Scott},
    title = {Three-dimensional computation of drift Alfv{\'{e}}n turbulence},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://doi.org/10.1088/0741-3335/39/10/010}{\textbf{39} 1635}},
	year = {(1997)},
}

@article{Ribeiro2008,
	author = {T. T. Ribeiro and B. Scott},
	title = {Gyrofluid turbulence studies of the effect of the poloidal position of an axisymmetric Debye sheath},
	journal = {Plasma Phys. Control. Fusion},
	volume =  {\href{https://doi.org/10.1088/0741-3335/50/5/055007}{\textbf{50} 055007}},
	year = {(2008)},
}

@article{Sykes2001,
    author = {A. Sykes and others},
    title = {First results from {MAST}},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/0029-5515/41/10/310}{\textbf{41} 1423}},
    year = {(2001)}
}

@article{Sun2015,
	author = {H. J. Sun and others},
	title = {Study of near scrape-off layer ({SOL}) temperature and density gradient lengths with Thomson scattering},
	journal = {Plasma Phys. Control. Fusion},
	volume =  {\href{https://doi.org/10.1088/0741-3335/57/12/125011}{\textbf{57} 125011}},
    year = {(2015)}
}

@book{Stangeby2000,
    title = {The Plasma Boundary of Magnetic Fusion Devices},
    author = {P. M. Stangeby},
    year = {2000},
    publisher= {IOP Publishing Ltd},
}

@article{Silvagni2020,
	author = {D. Silvagni and others},
	title = {{Scrape-off layer ({SOL}) power width scaling and correlation between {SOL} and pedestal gradients across L, I and H-mode plasmas at {ASDEX} Upgrade}},
	journal = {Plasma Phys. Control. Fusion},
	volume =  {\href{https://doi.org/10.1088/1361-6587/ab74e8}{\textbf{62} 045015}},
	year = {(2020)},
}

@article{Maurizio2017,
    author = {R. Maurizio and others},
    title = {{Divertor power load studies for attached L-mode single-null plasmas in {TCV}}},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/1741-4326/aa986b}{\textbf{58} 016052}},
	year={(2017)},
}

@article{Reimerdes2020,
    author = {H. Reimerdes and others},
    title = {Assessment of alternative divertor configurations as an exhaust solution for {DEMO}},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/1741-4326/ab8a6a}{\textbf{60} 066030}},
	year = {(2020)},
}

@article{Fernandez2022,
	author = {P. Rodriguez-Fernandez and others},
	title = {Overview of the {SPARC} physics basis towards the exploration of burning-plasma regimes in high-field, compact tokamaks},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/1741-4326/ac1654}{\textbf{62} 042003}},
	year = {(2020)},
}

@article{Giruzzi2017,
	author = {G. Giruzzi and others},
	title = {{Physics and operation oriented activities in preparation of the {JT}-60SA tokamak exploitation}},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/1741-4326/aa7962}{\textbf{57} 085001}},
	year = {(2020)},
}

@article{Campbell2016,
	author = {D.J. Campbell},
	title = {{The first fusion reactor: ITER}},
	journal = {Europhys. News},
	volume =  {\href{https://doi.org/10.1051/epn/2016504}{\textbf{47} 28}},
	year = {(2016)},
}

@book{Contessa2019,
	author = {G.M. Contessa and others},
	title = {{DTT-Divertor Tokamak Test Facility-Interim Design Report}},
	ISBN = {978-88-8286-378-4},
	publisher = {ENEA},
	year = {(2019)},
}

@article{Eich2013,
	author = {T. Eich and others},
	title = {Scaling of the tokamak near the scrape-off layer H-mode power width and implications for {ITER}},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/0029-5515/53/9/093031}{\textbf{53} 093031}},
	year = {(2013)},
}

@article{Chu2022,
	author = {X. Chu and P.H. Diamond and Z. Guo},
	title = {{SOL} width broadening by spreading of pedestal turbulence},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/1741-4326/ac4f9f}{\textbf{62} 066021}},
	year = {(2022)},
}

@article{Eich2020,
	author = {T. Eich and others},
	title = {{Turbulence driven widening of the near-{SOL} power width in {ASDEX} Upgrade H-Mode discharges}},
	journal = {Nucl. Fusion},
	volume =  {\href{https://doi.org/10.1088/1741-4326/ab7a66}{\textbf{60} 056016}},
	year = {(2020)},
}

@article{JET,
	author = {JET Design Group},
	title = {{The JET project - Preliminary description. (EUR-JET-R1)}},
	journal = {Culham Laboratory},
	year = {(1973)},
}


@article{Ran1989,
	author = {L. B. Ran and others},
	title = {Impurity accumulation in plasma regimes with high energy confinement},
	journal = {J. Nucl. Mater.},
	volume =  {\href{https://doi.org/10.1016/0022-3115(89)90254-7}{\textbf{162-164} 14}},
	year = {(1989)},
}

@article{Ricci2012,
	author = {P. Ricci and others},
	title = {{Simulation of plasma turbulence in scrape-off layer conditions: the GBS code, simulation results and code validation}},
	journal = {Plasma Phys. Control. Fusion},
	volume =  {\href{https://doi.org/10.1088/0741-3335/54/12/124047}{\textbf{54} 124047}},
	year = {(2012)},
}

@article{Rogers2013,
  title = {Low-Frequency Turbulence in a Linear Magnetized Plasma},
  author = {B. N. Rogers and P. Ricci},
  journal = {Phys. Rev. Lett.},
  volume =  {\href{https://doi.org/10.1103/PhysRevLett.104.225002}{\textbf{104} 225002}},
  year = {(2013)},
}

@article{Rogers2005,
    title = {Noncurvature-driven modes in a transport barrier},
    author = {Rogers,B. N.  and Dorland,W. },
    journal = {Phys. Plasmas},
    volume =  {\href{https://doi.org/10.1063/1.1928250}{\textbf{12} 062511}},
    year = {(2005)},
}

@article{Myra2016, 
    title={{Analytical and numerical study of the transverse Kelvin–Helmholtz instability in tokamak edge plasmas}},
    author={Myra, J. R. and D’Ippolito, D. A. and Russell, D. A. and Umansky, M. V. and Baver, D. A.},
    journal={J. Plasma Phys.},
    volume =  {\href{https://doi.org/10.1017/S0022377816000301}{\textbf{82} 905820210}},
    year = {(2016)},
}

@article{Happel2023,
    author = {T. Happel and others},
    title = {{Overview of initial negative triangularity plasma studies on the ASDEX Upgrade tokamak}},
    journal = {Nucl. Fusion},
    volume =  {\href{https://doi.org/10.1088/1741-4326/ac8563}{\textbf{63} 016002}},
    year = {(2023)},
}

@article{Ahn2006,
    author = {J-W. Ahn and G. F. Counsell and A. Kirk},
    title = {{L-mode SOL width scaling in the MAST spherical tokamak}},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://dx.doi.org/10.1088/0741-3335/48/8/003}{\textbf{48} 1077}},
    year = {(2006)},
}

@article{Brunner2018,
    author = {D. Brunner and B. LaBombard and A.Q. Kuang and J.L. Terry},
    title = {{High-resolution heat flux width measurements at reactor-level magnetic fields and observation of a unified width scaling across confinement regimes in the Alcator C-Mod tokamak}},
    journal = {Nucl. Fusion},
    volume =  {\href{https://dx.doi.org/10.1088/1741-4326/aad0d6}{\textbf{58} 094002}},
    year = {(2018)},
}

@article{Scarabosio2013,
    author = {A. Scarabosio and T. Eich and A. Herrmann and B. Sieglin},
    title = {{Outer target heat fluxes and power decay length scaling in L-mode plasmas at JET and AUG}},
    journal = {J. Nucl. Mater.},
    volume =  {\href{https://doi.org/10.1016/j.jnucmat.2013.01.086}{\textbf{438} S426-S430}},
    year = {(2013)},
}

@article{Reimerdes2022,
    author = {H. Reimerdes and others},
    title = {{Overview of the TCV tokamak experimental programme}},
    journal = {Nucl. Fusion},
    volume =  {\href{https://dx.doi.org/10.1088/1741-4326/ac369b}{\textbf{62} 042018}},
    year = {(2013)},
}

@article{Fevrier2018,
    author = {Février, O. and Theiler, C. and De Oliveira, H. and Labit, B. and Fedorczak, N. and Baillod, A.},
    title = {{Analysis of wall-embedded Langmuir probe signals in different conditions on the Tokamak à Configuration Variable}},
    journal = {Rev. Sci. Instrum.},
    volume =  {\href{https://doi.org/10.1063/1.5022459}{\textbf{89} 053502}},
    year = {(2018)},
}

@article{Oliveira2019,
    author = {De Oliveira, H. and Marmillod, P. and Theiler, C. and Chavan, R. and Février, O. and Labit, B. and Lavanchy, P. and Marlétaz, B. and Pitts, R. A. and TCV team},
    title = {{Langmuir probe electronics upgrade on the tokamak à configuration variable}},
    journal = {Rev. Sci. Instrum.},
    volume =  {\href{https://doi.org/10.1063/1.5108876}{\textbf{90} 083502}},
    year = {(2019)},
}

@article{Gorno2023,
    author = {S. Gorno and others},
    title = {{Power exhaust and core-divertor compatibility of the baffled snowflake divertor in TCV}},
    journal = {Plasma Phys. Control. Fusion},
    volume =  {\href{https://dx.doi.org/10.1088/1361-6587/acad26}{\textbf{65} 035004}},
    year = {(2023)},
}







